Gated Graph Recurrent Neural Networks

Graph processes exhibit a temporal structure determined by the sequence index and and a spatial structure determined by the graph support. To learn from graph processes, an information processing architecture must then be able to exploit both underlying structures. We introduce Graph Recurrent Neural Networks (GRNNs) as a general learning framework that achieves this goal by leveraging the notion of a recurrent hidden state together with graph signal processing (GSP). In the GRNN, the number of learnable parameters is independent of the length of the sequence and of the size of the graph, guaranteeing scalability. We prove that GRNNs are permutation equivariant and that they are stable to perturbations of the underlying graph support. To address the problem of vanishing gradients, we also put forward gated GRNNs with three different gating mechanisms: time, node and edge gates. In numerical experiments involving both synthetic and real datasets, time-gated GRNNs are shown to improve upon GRNNs in problems with long term dependencies, while node and edge gates help encode long range dependencies present in the graph. The numerical results also show that GRNNs outperform GNNs and RNNs, highlighting the importance of taking both the temporal and graph structures of a graph process into account.

==> abstract.tex <==
Graph processes consist of sequences of graph signals that vary in time on a static graph. They can be used to model data such as climate variables on weather station networks and seismic wave readings in a network of seismographs. Our objective is to introduce a permutation equivariant Graph Recurrent Neural Network (GRNN). GRNNs learn representations of graph processes by taking both their sequential structure and the underlying graph topology into account, while also keeping the number of parameters independent of the length of the sequence and of the size of the graph. The stability of GRNNs to graph perturbations is analyzed, and their architecture is extended to include three gating strategies, which address the problem of vanishing/exploding gradients over time and across paths of the graph. The advantages of the GRNN parametrization are demonstrated in a regression and a classification experiment, where GRNNs outperform both GNNs and RNNs, and time, node and edge gating yield gains in performance in different time and spatial correlation scenarios.

==> figures/AggregationCNNGS/AggregationCNNGSParam.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{4}
\def\Yscale{0.125}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{PathNodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {32} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {10} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.6}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {8}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {8}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {2}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {2}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {1.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.2*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.7*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/AggregationCNNGS/AggregationCNNGSParamGraph.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{GraphNodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {100} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {80/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.2}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {30}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {5}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {1}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {5}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {3}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {2*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.2*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {3*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/AggregationCNNGS/GraphNodePositions.tex <==
\def \posXarray {{
0.47, 0.22, 0.78, 0.09, 0.81, 
0.63, 0.90, 0.99, 0.77, 0.70, 0.01, 0.61, 0.55, 0.04, 0.72, 0.98, 0.68, 0.57, 0.26, 0.23, 0.28, 0.06, 0.85, 0.89, 0.98, 
0.88, 0.26, 0.02, 0.14, 0.17, 0.20, 0.01, 0.68, 0.77, 0.05, 0.60, 0.60, 0.04, 0.50, 0.05, 0.49, 0.38, 0.85, 0.48, 0.49, 
0.28, 0.26, 0.80, 0.84, 0.71, 0.36, 0.22, 0.33, 0.10, 0.99, 0.04, 0.66, 0.20, 0.91, 0.21, 0.04, 0.26, 0.16, 0.25, 0.68, 
0.89, 0.92, 0.25, 0.45, 0.77, 0.31, 0.99, 0.09, 0.41, 0.45, 0.63, 0.19, 0.28, 0.58, 0.28, 0.72, 0.25, 0.80, 0.26, 0.61, 
0.19, 0.16, 0.09, 0.32, 0.08, 0.39, 0.04, 0.93, 0.83, 0.72, 0.81, 0.38, 0.94, 0.42, 0.66, 0.88, 0.30, 0.77, 0.58, 0.68, 
%0.64, 0.09, 0.35, 0.30, 0.75, 0.44, 0.40, 0.47, 0.77, 0.29, 0.41, 0.64, 0.27, 0.18, 0.77, 0.98, 0.97, 0.05, 0.45, 0.28, 
%0.65, 0.30, 0.17, 0.69, 0.60, 0.22, 0.68, 0.05, 0.61, 0.50, 0.50, 0.46, 0.76, 0.13, 0.73, 0.53, 0.31, 0.66, 0.49, 0.63, 
%0.35, 0.24, 0.81, 0.75, 0.37, 0.58, 0.57, 0.48, 0.73, 0.89, 0.16, 0.62, 0.44, 0.53, 0.82, 0.80, 0.02, 0.92, 0.16, 0.12, 
%0.19, 0.66, 0.75, 0.48, 0.17, 0.49, 0.50, 0.02, 0.40, 0.70, 0.39, 0.20, 0.32, 0.52, 0.31, 0.76, 0.29, 0.51, 0.66, 0.80, 
%0.16, 0.65, 0.13, 0.63, 0.35, 0.44, 0.06, 0.87, 0.23, 0.43, 0.13, 0.56, 0.36, 0.45, 0.25, 0.61, 0.26, 0.29, 0.99, 0.04
}}

\def \posYarray {{
0.52, 0.18, 0.22, 0.83, 0.78, 
0.03, 0.61, 0.08, 0.86, 0.33, 0.64, 0.99, 0.43, 0.50, 0.63, 0.63, 0.40, 0.51, 0.22, 0.06, 0.03, 0.19, 0.18, 0.23, 0.16, 
0.21, 0.19, 0.12, 0.35, 0.06, 0.28, 0.76, 0.66, 0.25, 0.62, 0.13, 0.72, 0.98, 0.84, 0.40, 0.05, 0.25, 0.85, 0.22, 0.45, 
0.17, 0.10, 0.89, 0.43, 0.84, 0.12, 0.62, 0.64, 0.51, 0.78, 0.39, 0.67, 0.64, 0.32, 0.87, 0.81, 0.06, 0.05, 0.18, 0.62, 
0.79, 0.44, 0.87, 0.69, 0.59, 0.49, 0.86, 0.71, 0.64, 0.66, 0.13, 0.87, 0.96, 0.57, 0.53, 0.20, 0.99, 0.15, 0.48, 0.37, 
0.67, 0.35, 0.41, 0.71, 0.77, 0.95, 0.07, 0.07, 0.03, 0.40, 0.66, 0.82, 0.28, 0.50, 0.18, 0.65, 0.52, 0.24, 0.37, 0.67, 
%0.28, 0.78, 0.57, 0.60, 0.47, 0.67, 0.14, 0.06, 0.55, 0.10, 0.10, 0.19, 0.22, 0.82, 0.58, 0.48, 0.68, 0.87, 0.84, 0.69, 
%0.09, 0.88, 0.69, 0.81, 0.22, 0.11, 0.14, 0.22, 0.04, 0.77, 0.92, 0.92, 0.61, 0.38, 0.14, 0.81, 0.93, 0.17, 0.42, 0.30, 
%0.22, 0.39, 0.76, 0.79, 0.48, 0.74, 0.81, 0.39, 0.68, 0.54, 0.29, 0.48, 0.51, 0.45, 0.35, 0.31, 0.23, 0.09, 0.81, 0.76, 
%0.19, 0.30, 0.46, 0.13, 0.71, 0.81, 0.41, 0.10, 0.05, 0.86, 0.89, 0.95, 0.60, 0.17, 0.76, 0.03, 0.23, 0.49, 0.12, 0.28,
%0.94, 0.44, 0.39, 0.23, 0.25, 0.03, 0.59, 0.66, 0.40, 0.44, 0.02, 0.58, 0.02, 0.46, 0.02, 0.40, 0.57, 0.59, 0.56, 0.97
}}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/AggregationCNNGS/PathNodePositions.tex <==
\def \posXarray {{0.000, 0.516, 0.129, 0.258, 0.387, 0.645, 0.774, 0.903, 0.032, 0.065, 
0.097, 0.161, 0.194, 0.226, 0.290, 0.323, 0.355, 0.419, 0.452, 0.484, 
0.548, 0.581, 0.613, 0.677, 0.710, 0.742, 0.806, 0.839, 0.871, 0.935, 
0.968, 1.000, }}

\def \posYarray {{0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 
0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 
0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 
0.500, 0.500, }}

\input{../ToolsCNNGS/palettes/w3schools.tex}

==> figures/AggregationCNNGS/_fuse_hidden0002970600000022 <==
This is pdfTeX, Version 3.14159265-2.6-1.40.16 (TeX Live 2015/Debian) (preloaded format=pdflatex 2018.2.13)  26 MAR 2018 17:38
entering extended mode
 restricted \write18 enabled.
 %&-line parsing enabled.
**SelectionCNNGSLayer3Pool.tex
(./SelectionCNNGSLayer3Pool.tex
LaTeX2e <2016/02/01>
Babel <3.9q> and hyphenation patterns for 81 language(s) loaded.
(/usr/share/texlive/texmf-dist/tex/latex/standalone/standalone.cls
Document Class: standalone 2015/07/15 v1.2 Class to compile TeX sub-files stand
alone
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifluatex.sty
Package: ifluatex 2010/03/01 v1.3 Provides the ifluatex switch (HO)
Package ifluatex Info: LuaTeX not detected.
)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ifpdf.sty
Package: ifpdf 2011/01/30 v2.3 Provides the ifpdf switch (HO)
Package ifpdf Info: pdfTeX in PDF mode is detected.
)
(/usr/share/texlive/texmf-dist/tex/generic/ifxetex/ifxetex.sty
Package: ifxetex 2010/09/12 v0.6 Provides ifxetex conditional
)
(/usr/share/texlive/texmf-dist/tex/latex/xkeyval/xkeyval.sty
Package: xkeyval 2014/12/03 v2.7a package option processing (HA)

(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/xkvutils.tex
\XKV@toks=\toks14
\XKV@tempa@toks=\toks15

(/usr/share/texlive/texmf-dist/tex/generic/xkeyval/keyval.tex))
\XKV@depth=\count79
File: xkeyval.tex 2014/12/03 v2.7a key=value parser (HA)
))
\sa@internal=\count80
\c@sapage=\count81

(/usr/share/texlive/texmf-dist/tex/latex/standalone/standalone.cfg
File: standalone.cfg 2015/07/15 v1.2 Default configuration file for 'standalone
' class
)
(/usr/share/texlive/texmf-dist/tex/latex/base/article.cls
Document Class: article 2014/09/29 v1.4h Standard LaTeX document class
(/usr/share/texlive/texmf-dist/tex/latex/base/size10.clo
File: size10.clo 2014/09/29 v1.4h Standard LaTeX file (size option)
)
\c@part=\count82
\c@section=\count83
\c@subsection=\count84
\c@subsubsection=\count85
\c@paragraph=\count86
\c@subparagraph=\count87
\c@figure=\count88
\c@table=\count89
\abovecaptionskip=\skip41
\belowcaptionskip=\skip42
\bibindent=\dimen102
)
(/usr/share/texlive/texmf-dist/tex/latex/varwidth/varwidth.sty
Package: varwidth 2009/03/30 ver 0.92;  Variable-width minipages
\@vwid@box=\box26
\sift@deathcycles=\count90
\@vwid@loff=\dimen103
\@vwid@roff=\dimen104
)
\sa@box=\box27
)
(/usr/share/texlive/texmf-dist/tex/latex/xcolor/xcolor.sty
Package: xcolor 2007/01/21 v2.11 LaTeX color extensions (UK)

(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/color.cfg
File: color.cfg 2007/01/18 v1.5 color configuration of teTeX/TeXLive
)
Package xcolor Info: Driver file: pdftex.def on input line 225.

(/usr/share/texlive/texmf-dist/tex/latex/pdftex-def/pdftex.def
File: pdftex.def 2011/05/27 v0.06d Graphics/color for pdfTeX

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/infwarerr.sty
Package: infwarerr 2010/04/08 v1.3 Providing info/warning/error messages (HO)
)
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/ltxcmds.sty
Package: ltxcmds 2011/11/09 v1.22 LaTeX kernel commands for general use (HO)
)
\Gread@gobject=\count91
)
Package xcolor Info: Model `cmy' substituted by `cmy0' on input line 1337.
Package xcolor Info: Model `hsb' substituted by `rgb' on input line 1341.
Package xcolor Info: Model `RGB' extended on input line 1353.
Package xcolor Info: Model `HTML' substituted by `rgb' on input line 1355.
Package xcolor Info: Model `Hsb' substituted by `hsb' on input line 1356.
Package xcolor Info: Model `tHsb' substituted by `hsb' on input line 1357.
Package xcolor Info: Model `HSB' substituted by `hsb' on input line 1358.
Package xcolor Info: Model `Gray' substituted by `gray' on input line 1359.
Package xcolor Info: Model `wave' substituted by `hsb' on input line 1360.
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.tex
\pgfutil@everybye=\toks16
\pgfutil@tempdima=\dimen105
\pgfutil@tempdimb=\dimen106

(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-lists.t
ex)) (/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
\pgfutil@abb=\box28
(/usr/share/texlive/texmf-dist/tex/latex/ms/everyshi.sty
Package: everyshi 2001/05/15 v3.00 EveryShipout Package (MS)
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
Package: pgfrcs 2015/08/07 v3.0.1a (rcs-revision 1.31)
))
Package: pgf 2015/08/07 v3.0.1a (rcs-revision 1.15)

(/usr/share/texlive/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphicx.sty
Package: graphicx 2014/10/28 v1.0g Enhanced LaTeX Graphics (DPC,SPQR)

(/usr/share/texlive/texmf-dist/tex/latex/graphics/graphics.sty
Package: graphics 2016/01/03 v1.0q Standard LaTeX Graphics (DPC,SPQR)

(/usr/share/texlive/texmf-dist/tex/latex/graphics/trig.sty
Package: trig 2016/01/03 v1.10 sin cos tan (DPC)
)
(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/graphics.cfg
File: graphics.cfg 2010/04/23 v1.9 graphics configuration of TeX Live
)
Package graphics Info: Driver file: pdftex.def on input line 95.
)
\Gin@req@height=\dimen107
\Gin@req@width=\dimen108
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
Package: pgfsys 2014/07/09 v3.0.1a (rcs-revision 1.48)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
\pgfkeys@pathtoks=\toks17
\pgfkeys@temptoks=\toks18

(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.code.t
ex
\pgfkeys@tmptoks=\toks19
))
\pgf@x=\dimen109
\pgf@y=\dimen110
\pgf@xa=\dimen111
\pgf@ya=\dimen112
\pgf@xb=\dimen113
\pgf@yb=\dimen114
\pgf@xc=\dimen115
\pgf@yc=\dimen116
\w@pgf@writea=\write3
\r@pgf@reada=\read1
\c@pgf@counta=\count92
\c@pgf@countb=\count93
\c@pgf@countc=\count94
\c@pgf@countd=\count95
\t@pgf@toka=\toks20
\t@pgf@tokb=\toks21
\t@pgf@tokc=\toks22
 (/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg
File: pgf.cfg 2008/05/14  (rcs-revision 1.7)
)
Driver file for pgf: pgfsys-pdftex.def

(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.def
File: pgfsys-pdftex.def 2014/10/11  (rcs-revision 1.35)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-pdf.de
f
File: pgfsys-common-pdf.def 2013/10/10  (rcs-revision 1.13)
)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.code.
tex
File: pgfsyssoftpath.code.tex 2013/09/09  (rcs-revision 1.9)
\pgfsyssoftpath@smallbuffer@items=\count96
\pgfsyssoftpath@bigbuffer@items=\count97
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.code.
tex
File: pgfsysprotocol.code.tex 2006/10/16  (rcs-revision 1.4)
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
Package: pgfcore 2010/04/11 v3.0.1a (rcs-revision 1.7)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex
\pgfmath@dimen=\dimen117
\pgfmath@count=\count98
\pgfmath@box=\box29
\pgfmath@toks=\toks23
\pgfmath@stack@operand=\toks24
\pgfmath@stack@operation=\toks25
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.tex
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigonomet
ric.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.random.cod
e.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.comparison
.code.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round.code
.tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.code.
tex)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integerari
thmetics.code.tex)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex
\c@pgfmathroundto@lastzeros=\count99
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.code.te
x
File: pgfcorepoints.code.tex 2013/10/07  (rcs-revision 1.27)
\pgf@picminx=\dimen118
\pgf@picmaxx=\dimen119
\pgf@picminy=\dimen120
\pgf@picmaxy=\dimen121
\pgf@pathminx=\dimen122
\pgf@pathmaxx=\dimen123
\pgf@pathminy=\dimen124
\pgf@pathmaxy=\dimen125
\pgf@xx=\dimen126
\pgf@xy=\dimen127
\pgf@yx=\dimen128
\pgf@yy=\dimen129
\pgf@zx=\dimen130
\pgf@zy=\dimen131
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconstruct.
code.tex
File: pgfcorepathconstruct.code.tex 2013/10/07  (rcs-revision 1.29)
\pgf@path@lastx=\dimen132
\pgf@path@lasty=\dimen133
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage.code
.tex
File: pgfcorepathusage.code.tex 2014/11/02  (rcs-revision 1.24)
\pgf@shorten@end@additional=\dimen134
\pgf@shorten@start@additional=\dimen135
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.code.te
x
File: pgfcorescopes.code.tex 2015/05/08  (rcs-revision 1.46)
\pgfpic=\box30
\pgf@hbox=\box31
\pgf@layerbox@main=\box32
\pgf@picture@serial@count=\count100
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicstate.c
ode.tex
File: pgfcoregraphicstate.code.tex 2014/11/02  (rcs-revision 1.12)
\pgflinewidth=\dimen136
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransformation
s.code.tex
File: pgfcoretransformations.code.tex 2015/08/07  (rcs-revision 1.20)
\pgf@pt@x=\dimen137
\pgf@pt@y=\dimen138
\pgf@pt@temp=\dimen139
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.code.tex
File: pgfcorequick.code.tex 2008/10/09  (rcs-revision 1.3)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.code.t
ex
File: pgfcoreobjects.code.tex 2006/10/11  (rcs-revision 1.2)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathprocessing
.code.tex
File: pgfcorepathprocessing.code.tex 2013/09/09  (rcs-revision 1.9)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.code.te
x
File: pgfcorearrows.code.tex 2015/05/14  (rcs-revision 1.43)
\pgfarrowsep=\dimen140
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.code.tex
File: pgfcoreshade.code.tex 2013/07/15  (rcs-revision 1.15)
\pgf@max=\dimen141
\pgf@sys@shading@range@num=\count101
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.code.tex
File: pgfcoreimage.code.tex 2013/07/15  (rcs-revision 1.18)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.code.
tex
File: pgfcoreexternal.code.tex 2014/07/09  (rcs-revision 1.21)
\pgfexternal@startupbox=\box33
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.code.te
x
File: pgfcorelayers.code.tex 2013/07/18  (rcs-revision 1.7)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransparency.c
ode.tex
File: pgfcoretransparency.code.tex 2013/09/30  (rcs-revision 1.5)
)
(/usr/share/texlive/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.code.
tex
File: pgfcorepatterns.code.tex 2013/11/07  (rcs-revision 1.5)
)))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex
File: pgfmoduleshapes.code.tex 2014/03/21  (rcs-revision 1.35)
\pgfnodeparttextbox=\box34
) (/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.tex
File: pgfmoduleplot.code.tex 2015/08/03  (rcs-revision 1.13)
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-0-65
.sty
Package: pgfcomp-version-0-65 2007/07/03 v3.0.1a (rcs-revision 1.7)
\pgf@nodesepstart=\dimen142
\pgf@nodesepend=\dimen143
)
(/usr/share/texlive/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-1-18
.sty
Package: pgfcomp-version-1-18 2007/07/23 v3.0.1a (rcs-revision 1.1)
)) (/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/share/texlive/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex))
(/usr/share/texlive/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
Package: pgffor 2013/12/13 v3.0.1a (rcs-revision 1.25)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)
\pgffor@iter=\dimen144
\pgffor@skip=\dimen145
\pgffor@stack=\toks26
\pgffor@toks=\toks27
))
(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.code.tex
Package: tikz 2015/08/07 v3.0.1a (rcs-revision 1.151)

(/usr/share/texlive/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothandlers
.code.tex
File: pgflibraryplothandlers.code.tex 2013/08/31 v3.0.1a (rcs-revision 1.20)
\pgf@plot@mark@count=\count102
\pgfplotmarksize=\dimen146
)
\tikz@lastx=\dimen147
\tikz@lasty=\dimen148
\tikz@lastxsaved=\dimen149
\tikz@lastysaved=\dimen150
\tikzleveldistance=\dimen151
\tikzsiblingdistance=\dimen152
\tikz@figbox=\box35
\tikz@figbox@bg=\box36
\tikz@tempbox=\box37
\tikz@tempbox@bg=\box38
\tikztreelevel=\count103
\tikznumberofchildren=\count104
\tikznumberofcurrentchild=\count105
\tikz@fig@count=\count106

(/usr/share/texlive/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.code.tex
File: pgfmodulematrix.code.tex 2013/09/17  (rcs-revision 1.8)
\pgfmatrixcurrentrow=\count107
\pgfmatrixcurrentcolumn=\count108
\pgf@matrix@numberofcolumns=\count109
)
\tikz@expandcount=\count110

(/usr/share/texlive/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tik
zlibrarytopaths.code.tex
File: tikzlibrarytopaths.code.tex 2008/06/17 v3.0.1a (rcs-revision 1.2)
)))
(/usr/share/texlive/texmf-dist/tex/latex/subfigure/subfigure.sty
Package: subfigure 2002/03/15 v2.1.5 subfigure package
\subfigtopskip=\skip43
\subfigcapskip=\skip44
\subfigcaptopadj=\dimen153
\subfigbottomskip=\skip45
\subfigcapmargin=\dimen154
\subfiglabelskip=\skip46
\c@subfigure=\count111
\c@lofdepth=\count112
\c@subtable=\count113
\c@lotdepth=\count114

****************************************
* Local config file subfigure.cfg used *
****************************************
(/usr/share/texlive/texmf-dist/tex/latex/subfigure/subfigure.cfg)
\subfig@top=\skip47
\subfig@bottom=\skip48
)
(./SelectionCNNGSLayer3Pool.aux)
\openout1 = `SelectionCNNGSLayer3Pool.aux'.

LaTeX Font Info:    Checking defaults for OML/cmm/m/it on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for T1/cmr/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for OT1/cmr/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for OMS/cmsy/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for OMX/cmex/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.
LaTeX Font Info:    Checking defaults for U/cmr/m/n on input line 6.
LaTeX Font Info:    ... okay on input line 6.

(/usr/share/texlive/texmf-dist/tex/context/base/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
\scratchcounter=\count115
\scratchdimen=\dimen155
\scratchbox=\box39
\nofMPsegments=\count116
\nofMParguments=\count117
\everyMPshowfont=\toks28
\MPscratchCnt=\count118
\MPscratchDim=\dimen156
\MPnumerator=\count119
\makeMPintoPDFobject=\count120
\everyMPtoPDFconversion=\toks29
) ABD: EveryShipout initializing macros
(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/pdftexcmds.sty
Package: pdftexcmds 2011/11/29 v0.20 Utility functions of pdfTeX for LuaTeX (HO
)
Package pdftexcmds Info: LuaTeX not detected.
Package pdftexcmds Info: \pdf@primitive is available.
Package pdftexcmds Info: \pdf@ifprimitive is available.
Package pdftexcmds Info: \pdfdraftmode found.
)
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/epstopdf-base.sty
Package: epstopdf-base 2010/02/09 v2.5 Base part for package epstopdf

(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/grfext.sty
Package: grfext 2010/08/19 v1.1 Manage graphics extensions (HO)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/kvdefinekeys.sty
Package: kvdefinekeys 2011/04/07 v1.3 Define keys (HO)
))
(/usr/share/texlive/texmf-dist/tex/latex/oberdiek/kvoptions.sty
Package: kvoptions 2011/06/30 v3.11 Key value format for package options (HO)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/kvsetkeys.sty
Package: kvsetkeys 2012/04/25 v1.16 Key value parser (HO)

(/usr/share/texlive/texmf-dist/tex/generic/oberdiek/etexcmds.sty
Package: etexcmds 2011/02/16 v1.5 Avoid name clashes with e-TeX commands (HO)
Package etexcmds Info: Could not find \expanded.
(etexcmds)             That can mean that you are not using pdfTeX 1.50 or
(etexcmds)             that some package has redefined \expanded.
(etexcmds)             In the latter case, load this package earlier.
)))
Package grfext Info: Graphics extension search list:
(grfext)             [.png,.pdf,.jpg,.mps,.jpeg,.jbig2,.jb2,.PNG,.PDF,.JPG,.JPE
G,.JBIG2,.JB2,.eps]
(grfext)             \AppendGraphicsExtensions on input line 452.

(/usr/share/texlive/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg
File: epstopdf-sys.cfg 2010/07/13 v1.3 Configuration of (r)epstopdf for TeX Liv
e
))
(./SelectionCNNGSParam.tex (../ToolsCNNGS/DrawFeatures.tex)
(../ToolsCNNGS/ChooseNodeColor.tex) (../ToolsCNNGS/DrawGraphNodes.tex)
(../ToolsCNNGS/DrawGraphEdges.tex (../ToolsCNNGS/AuxMacrosDrawEdges.tex))
\pgf@layerbox@NodeLayer=\box40
\pgf@layerboxsaved@NodeLayer=\box41
\pgf@layerbox@EdgeLayer=\box42
\pgf@layerboxsaved@EdgeLayer=\box43
\pgf@layerbox@GNNLayerLayer=\box44
\pgf@layerboxsaved@GNNLayerLayer=\box45

(./NodePositions.tex))
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
Missing character: There is no ; in font nullfont!
LaTeX Font Info:    External font `cmex10' loaded for size
(Font)              <7> on input line 72.
LaTeX Font Info:    External font `cmex10' loaded for size
(Font)              <5> on input line 72.
 [1

] (./SelectionCNNGSLayer3Pool.aux) ) 
Here is how much of TeX's memory you used:
 12480 strings out of 493029
 251718 string characters out of 6136234
 370574 words of memory out of 5000000
 15781 multiletter control sequences out of 15000+600000
 3640 words of font info for 14 fonts, out of 8000000 for 9000
 1141 hyphenation exceptions out of 8191
 55i,10n,66p,427b,857s stack positions out of 5000i,500n,10000p,200000b,80000s

Output written on SelectionCNNGSLayer3Pool.pdf (1 page, 7393 bytes).
PDF statistics:
 11 PDF objects out of 1000 (max. 8388607)
 7 compressed objects within 1 object stream
 0 named destinations out of 1000 (max. 500000)
 13 words of extra memory for PDF output out of 10000 (max. 10000000)



==> figures/AggregationCNNGS/_fuse_hidden0002970700000021 <==
\relax 


==> figures/RegularCNN/DrawGraphNodes.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodes}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired
      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position 
   \clip (-0.1+\XposO,-0.2+\YposO) rectangle 
   		(\widthI+0.2-0.1+\XposO, 
   		\heightI+0.3-0.1+\YposO);
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity]    % Node opacity
             (\posX cm, \posY cm)            % Node position
             circle (\localNodeSize pt);     % Node size

\end{pgfonlayer}       
}
}


==> figures/RegularCNN/DrawGraphNodesR.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodesR}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired
      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position 
     \clip (-0.1+\XposO,-0.1+\YposO) rectangle 
   		(\widthI+0.2-0.1+\XposO, 
   		\heightI+0.2-0.1+\YposO);
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity,    % Node opacity
             rounded corners]
             (\posX cm - \localNodeSize pt, \posY cm - \localNodeSize pt)            % Node position
             rectangle (\posX cm + \localNodeSize pt, \posY cm + \localNodeSize pt);     % Node size

\end{pgfonlayer}       
}
}


==> figures/RegularCNN/RegularCNNParamLayer1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{4}
\def\Yscale{0.125}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphNodesR.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{RegularNodePositionsLayer1.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {16} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {40/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.01}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {8}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {8}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {0.57*\Radius}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {1.25*\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {4}                  % Number of nodes sample
\pgfmathsetmacro \twoNrPooledNodes       {4}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {1.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.3*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.2*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/RegularCNN/RegularCNNParamLayer2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{4}
\def\Yscale{1}

\def\XposO{0.267*\Xscale} % X position of first node (Origin)
\def\YposO{0.5*\Yscale} % Y position of first node (Origin)
\def\widthI{0.733*\Xscale-\XposO} % Width of image
\def\heightI{0.5*\Yscale-\YposO} % Height of image

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{DrawGraphNodes.tex}
\input{DrawGraphNodesR.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{RegularNodePositionsLayer2.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {8} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {20} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {8}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {8}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {2}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {2}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {1.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.2*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/RegularCNN/RegularCNNParamLayer3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{4}
\def\Yscale{0.125}

\def\XposO{0.455*\Xscale} % X position of first node (Origin)
\def\YposO{0.5*\Yscale} % Y position of first node (Origin)
\def\widthI{0.545*\Xscale-\XposO} % Width of image
\def\heightI{0.5*\Yscale-\YposO} % Height of image

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{DrawGraphNodes.tex}
\input{DrawGraphNodesR.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{RegularNodePositionsLayer3.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {2} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {50} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {2}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {2}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {2}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {2}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {4.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.25*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {0.35*\LargeConvSize} % Size of large1 convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/RegularCNN/RegularNodePositionsLayer1.tex <==
\def \posXarray {{
0.000,
0.133,
0.267, 
0.400, 
0.533, 
0.667,
0.800,  
0.933, 
0.067, 
0.200, 
0.333, 
0.467, 
0.600, 
0.733, 
0.867,   
1.000, }}

\def \posYarray {{0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 0.500, 
0.500, 0.500, 0.500, 0.500, 0.500, 0.500, }}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/RegularCNN/RegularNodePositionsLayer2.tex <==
\def \posXarray {{
0.267,
0.533, 
0.333, 
0.400, 
0.467, 
0.600, 
0.667,
0.733, 
 }}

\def \posYarray {{ 0.500, 0.500, 
0.500, 0.500, 0.500, 0.500, 0.500, 0.500, }}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/RegularCNN/RegularNodePositionsLayer3.tex <==
\def \posXarray {{
0.455,
0.545,
}}

\def \posYarray {{0.5,
0.5,
}}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/RegularCNNGS/RegularCNNGSParam.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphNodesR.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{RegularNodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {96} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {40/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {12}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {12}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {1.5*\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {2}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {2}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {3*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {2.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {4*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {3*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/RegularCNNGS/RegularNodePositions.tex <==
\def \posXarray {{0.364, 0.636,
0.091, 0.091, 0.091, 0.364, 0.364, 0.636, 0.636, 0.909, 
0.909, 0.909, 0.000, 0.000, 0.000, 0.000, 0.000, 0.000, 0.000, 0.000, 
0.091, 0.091, 0.091, 0.091, 0.091, 0.182, 0.182, 0.182, 0.182, 0.182, 
0.182, 0.182, 0.182, 0.273, 0.273, 0.273, 0.273, 0.273, 0.273, 0.273, 
0.273, 0.364, 0.364, 0.364, 0.364, 0.364, 0.455, 0.455, 0.455, 0.455, 
0.455, 0.455, 0.455, 0.455, 0.545, 0.545, 0.545, 0.545, 0.545, 0.545, 
0.545, 0.545, 0.636, 0.636, 0.636, 0.636, 0.636, 0.727, 0.727, 0.727, 
0.727, 0.727, 0.727, 0.727, 0.727, 0.818, 0.818, 0.818, 0.818, 0.818, 
0.818, 0.818, 0.818, 0.909, 0.909, 0.909, 0.909, 0.909, 1.000, 1.000, 
1.000, 1.000, 1.000, 1.000, 1.000, 1.000, }}

\def \posYarray {{0.571, 0.571,
0.143, 0.571, 1.000, 0.143, 1.000, 0.143, 1.000, 0.143, 
0.571, 1.000, 0.000, 0.143, 0.286, 0.429, 0.571, 0.714, 0.857, 1.000, 
0.000, 0.286, 0.429, 0.714, 0.857, 0.000, 0.143, 0.286, 0.429, 0.571, 
0.714, 0.857, 1.000, 0.000, 0.143, 0.286, 0.429, 0.571, 0.714, 0.857, 
1.000, 0.000, 0.286, 0.429, 0.714, 0.857, 0.000, 0.143, 0.286, 0.429, 
0.571, 0.714, 0.857, 1.000, 0.000, 0.143, 0.286, 0.429, 0.571, 0.714, 
0.857, 1.000, 0.000, 0.286, 0.429, 0.714, 0.857, 0.000, 0.143, 0.286, 
0.429, 0.571, 0.714, 0.857, 1.000, 0.000, 0.143, 0.286, 0.429, 0.571, 
0.714, 0.857, 1.000, 0.000, 0.286, 0.429, 0.714, 0.857, 0.000, 0.143, 
0.286, 0.429, 0.571, 0.714, 0.857, 1.000, }}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/SelectionCNNGS/NodePositions.tex <==
\def \posXarray {{
0.47, 0.22, 0.78, 0.09, 0.81, 
0.63, 0.90, 0.99, 0.77, 0.70, 0.01, 0.61, 0.55, 0.04, 0.72, 0.98, 0.68, 0.57, 0.26, 0.23, 0.28, 0.06, 0.85, 0.89, 0.98, 
0.88, 0.26, 0.02, 0.14, 0.17, 0.20, 0.01, 0.68, 0.77, 0.05, 0.60, 0.60, 0.04, 0.50, 0.05, 0.49, 0.38, 0.85, 0.48, 0.49, 
0.28, 0.26, 0.80, 0.84, 0.71, 0.36, 0.22, 0.33, 0.10, 0.99, 0.04, 0.66, 0.20, 0.91, 0.21, 0.04, 0.26, 0.16, 0.25, 0.68, 
0.89, 0.92, 0.25, 0.45, 0.77, 0.31, 0.99, 0.09, 0.41, 0.45, 0.63, 0.19, 0.28, 0.58, 0.28, 0.72, 0.25, 0.80, 0.26, 0.61, 
0.19, 0.16, 0.09, 0.32, 0.08, 0.39, 0.04, 0.93, 0.83, 0.72, 0.81, 0.38, 0.94, 0.42, 0.66, 0.88, 0.30, 0.77, 0.58, 0.68, 
%0.64, 0.09, 0.35, 0.30, 0.75, 0.44, 0.40, 0.47, 0.77, 0.29, 0.41, 0.64, 0.27, 0.18, 0.77, 0.98, 0.97, 0.05, 0.45, 0.28, 
%0.65, 0.30, 0.17, 0.69, 0.60, 0.22, 0.68, 0.05, 0.61, 0.50, 0.50, 0.46, 0.76, 0.13, 0.73, 0.53, 0.31, 0.66, 0.49, 0.63, 
%0.35, 0.24, 0.81, 0.75, 0.37, 0.58, 0.57, 0.48, 0.73, 0.89, 0.16, 0.62, 0.44, 0.53, 0.82, 0.80, 0.02, 0.92, 0.16, 0.12, 
%0.19, 0.66, 0.75, 0.48, 0.17, 0.49, 0.50, 0.02, 0.40, 0.70, 0.39, 0.20, 0.32, 0.52, 0.31, 0.76, 0.29, 0.51, 0.66, 0.80, 
%0.16, 0.65, 0.13, 0.63, 0.35, 0.44, 0.06, 0.87, 0.23, 0.43, 0.13, 0.56, 0.36, 0.45, 0.25, 0.61, 0.26, 0.29, 0.99, 0.04
}}

\def \posYarray {{
0.52, 0.18, 0.22, 0.83, 0.78, 
0.03, 0.61, 0.08, 0.86, 0.33, 0.64, 0.99, 0.43, 0.50, 0.63, 0.63, 0.40, 0.51, 0.22, 0.06, 0.03, 0.19, 0.18, 0.23, 0.16, 
0.21, 0.19, 0.12, 0.35, 0.06, 0.28, 0.76, 0.66, 0.25, 0.62, 0.13, 0.72, 0.98, 0.84, 0.40, 0.05, 0.25, 0.85, 0.22, 0.45, 
0.17, 0.10, 0.89, 0.43, 0.84, 0.12, 0.62, 0.64, 0.51, 0.78, 0.39, 0.67, 0.64, 0.32, 0.87, 0.81, 0.06, 0.05, 0.18, 0.62, 
0.79, 0.44, 0.87, 0.69, 0.59, 0.49, 0.86, 0.71, 0.64, 0.66, 0.13, 0.87, 0.96, 0.57, 0.53, 0.20, 0.99, 0.15, 0.48, 0.37, 
0.67, 0.35, 0.41, 0.71, 0.77, 0.95, 0.07, 0.07, 0.03, 0.40, 0.66, 0.82, 0.28, 0.50, 0.18, 0.65, 0.52, 0.24, 0.37, 0.67, 
%0.28, 0.78, 0.57, 0.60, 0.47, 0.67, 0.14, 0.06, 0.55, 0.10, 0.10, 0.19, 0.22, 0.82, 0.58, 0.48, 0.68, 0.87, 0.84, 0.69, 
%0.09, 0.88, 0.69, 0.81, 0.22, 0.11, 0.14, 0.22, 0.04, 0.77, 0.92, 0.92, 0.61, 0.38, 0.14, 0.81, 0.93, 0.17, 0.42, 0.30, 
%0.22, 0.39, 0.76, 0.79, 0.48, 0.74, 0.81, 0.39, 0.68, 0.54, 0.29, 0.48, 0.51, 0.45, 0.35, 0.31, 0.23, 0.09, 0.81, 0.76, 
%0.19, 0.30, 0.46, 0.13, 0.71, 0.81, 0.41, 0.10, 0.05, 0.86, 0.89, 0.95, 0.60, 0.17, 0.76, 0.03, 0.23, 0.49, 0.12, 0.28,
%0.94, 0.44, 0.39, 0.23, 0.25, 0.03, 0.59, 0.66, 0.40, 0.44, 0.02, 0.58, 0.02, 0.46, 0.02, 0.40, 0.57, 0.59, 0.56, 0.97
}}

\input{../ToolsCNNGS/palettes/w3schools.tex}


==> figures/SelectionCNNGS/SelectionCNNGSParam.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{../ToolsCNNGS/DrawFeatures.tex}
\input{../ToolsCNNGS/ChooseNodeColor.tex}
\input{../ToolsCNNGS/DrawGraphNodes.tex}
\input{../ToolsCNNGS/DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{NodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {100} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {80/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {30}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {5}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)
\pgfmathsetmacro \onefeatures         {3}       % Number of features in first layer

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {5}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {3}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {1.5*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.2*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \twofeatures            {6}       % Number of features in second layer

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.7*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.5*\LargeConvSize} % Size of large convolution circles (pooling)
\pgfmathsetmacro \threefeatures            {10}       % Number of features in third layer


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/graph_drawing_experiments/AuxMacrosDrawEdges.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro for computing distance between 2 points

\newcommand{\CalculateDistance}[2]
{
   \pgfmathsetmacro\Distance{ sqrt(     (#1)^2 +    (#2)^2 ) }; % Calculates 2-norm distance
%  \pgfmathsetmacro\Distance{      abs( (#1)   + abs(#2)   ) }; % Calculates 1-norm distance. May be faster
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro to get coordniates of a node
\makeatletter
\newcommand{\GetTikzXY}[3]{ 
    \tikz@scan@one@point\pgfutil@firstofone#1\relax
    \edef#2{\the\pgf@x}
    \edef#3{\the\pgf@y}
}
\makeatother



==> figures/graph_drawing_experiments/ChooseNodeColor.tex <==

% Macro for selecting node's color based on positions. The macro is not used in the final version. 
% Accepts as argument the (x,y) coordinate of the node.
% Returns the custom color currentcolor that can be used in color commands.

\newcommand{\ChooseNodeColor}[2]
{   
    % Store arguments of the function in readable variables
    \def\Xhere{#1}      
    \def\Yhere{#1}
    % Compute a color scale
    \pgfmathsetmacro{\thecurrentcolor}
                    { 0.8*exp( - 0.6*(abs(\Xhere-0.5) + abs(\Yhere-0.5)) }
    % Assign color scale according to colormap (Grayscale in current configuration}
    \definecolor{CurrentColor}{rgb}{\thecurrentcolor,\thecurrentcolor,\thecurrentcolor}
}



%\def\colors{{"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", 
%             "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%             "E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", 
%             "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%             "D5EAE7", "F3ELEB", "F6C4E1", "F79CD4"}} 
%
%\pgfmathsetmacro{\thecurrentcolor}{\colors[random(0,20)]}
%\definecolor{currentcolor}{HTML}{\thecurrentcolor}


==> figures/graph_drawing_experiments/DrawFeatures.tex <==

% Macro to draw a stack of features. 
% The first two parameters are the positions of the front feature. 
% The third and fourth two are the x and y offsets of subsequent features. 
% The fifth and sixth are the size of the features 
% The seventh parameter is the number of features
% The eight is the color of the feature plane

\newcommand{\DrawFeatures}[8]
{
   \pgfmathsetmacro\NumberFeatures {#7}    % The numb er of features is in the seventh parameter
   \foreach \i in {\NumberFeatures,...,1}  % Repeat number of features. Sweep backwards
   {
      \pgfmathsetmacro\FeaturePosX {(#3)*(\i-1)} % Offset x
      \pgfmathsetmacro\FeaturePosY {(#4)*(\i-1)} % Offset y     
      \path    (#1,           #2)          % Start position
            ++ (\FeaturePosX,\FeaturePosY) % Advance as per offset
       node[ draw, 
             rectangle, 
             black!70,
             anchor         = south west,
             fill           = #8, 
             minimum width  = #5,
             minimum height = #6    ]  {} ;
   }
}


==> figures/graph_drawing_experiments/DrawGraphEdges.tex <==
% Command to draw edges of a graph. The macro assumes that nodes have been 
% placed and that they have received tikZ labels of the form (a1), (a2), ..., (aN)
% This can be accomplished by loading the file DrawGraphNodes.tex:
%    \input{DrawGraphNodes.tex}
% and calling the macro DrawGraphNodes. The statement below draws nodes of a
% graph with 10 nodes and small circles for nodes:
%    \DrawGraphNodes {1}    % Start node
%                    {10}   % End node 
%                    {5}    % Node size
%                    {1}    % Opacity
%                    {0}    % X offset
%                    {0}    % Y offset

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    NrNodes: Number of nodes the graph has
%    Connectivity radius: How far aways to connect nodes  
%    Edge Color: A valid color to draw edges. E.g., gray!20.
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Load macros to get coordinate points and calculate distances
%
\input{AuxMacrosDrawEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphEdges}[7]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNrNodes     {#3}
\pgfmathsetmacro\localRadius      {#4}
\pgfmathsetmacro\localEdgeColor   {#5}
\pgfmathsetmacro\localOffsetX     {#6}
\pgfmathsetmacro\localOffsetY     {#7}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin loop for drawing graph edges. 
%% We sweep from \localStartNode to NrNodes drawing edges
%%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Draw node connections. We sweep through all nodes and check if they are close to \i
   % If the nodes are close, we draw an edge.
   \begin{pgfonlayer}{EdgeLayer} % Edges are drawn in the edge layer
      \GetTikzXY{(a\i)}{\NodePosX}{\NodePosY}; % Get coordinates of current node (node i)
      \pgfmathsetmacro\PreviousNode{\i -1} % A pgf technicality. Need to store index of previous node (\i-1)
      \foreach \j in {1,...,\localNrNodes} % Start loop sweeping through previous nodes
      {
         \GetTikzXY{(a\j)}{\OtherNodePosX}{\OtherNodePosY}; % Coordinates of the other node (node j)
         \CalculateDistance{\NodePosX-\OtherNodePosX}
                           {\NodePosY-\OtherNodePosY}; % Calculate distance between nodes i and j
         \ifdim \Distance cm < \localRadius cm % Check the nodes are close. 
            \draw[\localEdgeColor] (a\i) -- (a\j); %If they are close, draw and edge
         \fi 
      } % Close inner loop sweeping through previous nodes
   \end{pgfonlayer}      
} % Close main loop sweeping through nodes
}
 

==> figures/graph_drawing_experiments/DrawGraphNodes.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodes}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired

      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position   
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity]    % Node opacity
             (\posX cm, \posY cm)            % Node position
             circle (\localNodeSize pt);     % Node size
\end{pgfonlayer}       
}
}


==> figures/graph_drawing_experiments/NodePositions.tex <==
\def \posXarray {{
0.47, 0.22, 0.78, 0.09, 0.81, 
0.63, 0.90, 0.99, 0.77, 0.70, 0.01, 0.61, 0.55, 0.04, 0.72, 0.98, 0.68, 0.57, 0.26, 0.23, 0.28, 0.06, 0.85, 0.89, 0.98, 
0.88, 0.26, 0.02, 0.14, 0.17, 0.20, 0.01, 0.68, 0.77, 0.05, 0.60, 0.60, 0.04, 0.50, 0.05, 0.49, 0.38, 0.85, 0.48, 0.49, 
0.28, 0.26, 0.80, 0.84, 0.71, 0.36, 0.22, 0.33, 0.10, 0.99, 0.04, 0.66, 0.20, 0.91, 0.21, 0.04, 0.26, 0.16, 0.25, 0.68, 
0.89, 0.92, 0.25, 0.45, 0.77, 0.31, 0.99, 0.09, 0.41, 0.45, 0.63, 0.19, 0.28, 0.58, 0.28, 0.72, 0.25, 0.80, 0.26, 0.61, 
0.19, 0.16, 0.09, 0.32, 0.08, 0.39, 0.04, 0.93, 0.83, 0.72, 0.81, 0.38, 0.94, 0.42, 0.66, 0.88, 0.30, 0.77, 0.58, 0.68, 
%0.64, 0.09, 0.35, 0.30, 0.75, 0.44, 0.40, 0.47, 0.77, 0.29, 0.41, 0.64, 0.27, 0.18, 0.77, 0.98, 0.97, 0.05, 0.45, 0.28, 
%0.65, 0.30, 0.17, 0.69, 0.60, 0.22, 0.68, 0.05, 0.61, 0.50, 0.50, 0.46, 0.76, 0.13, 0.73, 0.53, 0.31, 0.66, 0.49, 0.63, 
%0.35, 0.24, 0.81, 0.75, 0.37, 0.58, 0.57, 0.48, 0.73, 0.89, 0.16, 0.62, 0.44, 0.53, 0.82, 0.80, 0.02, 0.92, 0.16, 0.12, 
%0.19, 0.66, 0.75, 0.48, 0.17, 0.49, 0.50, 0.02, 0.40, 0.70, 0.39, 0.20, 0.32, 0.52, 0.31, 0.76, 0.29, 0.51, 0.66, 0.80, 
%0.16, 0.65, 0.13, 0.63, 0.35, 0.44, 0.06, 0.87, 0.23, 0.43, 0.13, 0.56, 0.36, 0.45, 0.25, 0.61, 0.26, 0.29, 0.99, 0.04
}}

\def \posYarray {{
0.52, 0.18, 0.22, 0.83, 0.78, 
0.03, 0.61, 0.08, 0.86, 0.33, 0.64, 0.99, 0.43, 0.50, 0.63, 0.63, 0.40, 0.51, 0.22, 0.06, 0.03, 0.19, 0.18, 0.23, 0.16, 
0.21, 0.19, 0.12, 0.35, 0.06, 0.28, 0.76, 0.66, 0.25, 0.62, 0.13, 0.72, 0.98, 0.84, 0.40, 0.05, 0.25, 0.85, 0.22, 0.45, 
0.17, 0.10, 0.89, 0.43, 0.84, 0.12, 0.62, 0.64, 0.51, 0.78, 0.39, 0.67, 0.64, 0.32, 0.87, 0.81, 0.06, 0.05, 0.18, 0.62, 
0.79, 0.44, 0.87, 0.69, 0.59, 0.49, 0.86, 0.71, 0.64, 0.66, 0.13, 0.87, 0.96, 0.57, 0.53, 0.20, 0.99, 0.15, 0.48, 0.37, 
0.67, 0.35, 0.41, 0.71, 0.77, 0.95, 0.07, 0.07, 0.03, 0.40, 0.66, 0.82, 0.28, 0.50, 0.18, 0.65, 0.52, 0.24, 0.37, 0.67, 
%0.28, 0.78, 0.57, 0.60, 0.47, 0.67, 0.14, 0.06, 0.55, 0.10, 0.10, 0.19, 0.22, 0.82, 0.58, 0.48, 0.68, 0.87, 0.84, 0.69, 
%0.09, 0.88, 0.69, 0.81, 0.22, 0.11, 0.14, 0.22, 0.04, 0.77, 0.92, 0.92, 0.61, 0.38, 0.14, 0.81, 0.93, 0.17, 0.42, 0.30, 
%0.22, 0.39, 0.76, 0.79, 0.48, 0.74, 0.81, 0.39, 0.68, 0.54, 0.29, 0.48, 0.51, 0.45, 0.35, 0.31, 0.23, 0.09, 0.81, 0.76, 
%0.19, 0.30, 0.46, 0.13, 0.71, 0.81, 0.41, 0.10, 0.05, 0.86, 0.89, 0.95, 0.60, 0.17, 0.76, 0.03, 0.23, 0.49, 0.12, 0.28,
%0.94, 0.44, 0.39, 0.23, 0.25, 0.03, 0.59, 0.66, 0.40, 0.44, 0.02, 0.58, 0.02, 0.46, 0.02, 0.40, 0.57, 0.59, 0.56, 0.97
}}


\def \NodeColors{{
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
}} 


==> figures/graph_drawing_experiments/mainSelectionGNNParam.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale for the picture
\def \myfactor{2.7}
\def \myunit{\myfactor cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Import functions
\input{DrawFeatures.tex}
\input{ChooseNodeColor.tex}
\input{DrawGraphNodes.tex}
\input{DrawGraphEdges.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Declare pgf layers
\pgfdeclarelayer{NodeLayer}
\pgfdeclarelayer{EdgeLayer}
\pgfdeclarelayer{GNNLayerLayer}
\pgfsetlayers   {GNNLayerLayer,EdgeLayer,NodeLayer,main}

% Load coordinates. File loads arrays \posXarray and \posYarray with nodes coordinates
% There is a maximum of 200 points in the array.
\input{NodePositions.tex}

% Define parameters of the graph: nr of nodes in the graph and connectivity radius 
\pgfmathsetmacro \NrNodes             {20} % Number of nodes in the graph
\pgfmathsetmacro \Radius              {80/sqrt{\NrNodes}} % Connectivity radius of the graph

% Define aesthetics of nodes: Node sizes and opacity
\pgfmathsetmacro \NodeSize            {0.8}     % Size of a node
\pgfmathsetmacro \ConvOpacity         {0.3}     % Opacity of convolution circles
\pgfmathsetmacro \SampleOpacity       {0.1}     % Opacity of nodes that are not sampled

% Define parameters of plots for layer 1: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \NrSampledNodes      {30}      % Number of nodes sampled
\pgfmathsetmacro \NrPooledNodes       {5}       % Number of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \ConvSize            {3.7}     % Size of convolution circles
\pgfmathsetmacro \LargeConvSize       {\Radius} % Size of large convolution circles (pooling stage)

% Define parameters of plots for layer 2: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \twoNrSampledNodes      {5}                  % Number of nodes sampled
\pgfmathsetmacro \twoNrPooledNodes       {3}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \twoConvSize            {2.7*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \twoLargeConvSize       {1.3*\LargeConvSize} % Size of large convolution circles (pooling)

% Define parameters of plots for layer 3: nr of nodes sampled and pooled. convolution and pooling circle sizes
\pgfmathsetmacro \threeNrSampledNodes      {1}                  % Number of nodes sampled
\pgfmathsetmacro \threeNrPooledNodes       {1}                  % Nr of nodes to illustrate pooling neighborhood
\pgfmathsetmacro \threeConvSize            {2.7*\ConvSize}      % Size of convolution circles
\pgfmathsetmacro \threeLargeConvSize       {1.3*\LargeConvSize} % Size of large convolution circles (pooling)


% Define color aesthetics: Colors for edges and feature planes. Colors for nodes are in ChooseNodeColor.tex
\definecolor{EdgeColor}{rgb}{0.75,0.75,0.75}
\definecolor{LightEdgeColor}{rgb}{0.92,0.92,0.92}
\definecolor{DarkEdgeColor}{rgb}{0.6,0.6,0.6}
\definecolor{FeaturePlaneColor}{RGB}{240,240,240}


==> figures/graph_drawing_experiments/old/DrawGraph.tex <==
% Command to draw a random graph. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The Edge color is hard coded to light gray
% The size and shape of the node is also hard coded. They are 5pt circles

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The parameters passed to the macro are, in order: 
%    Number of nodes, 
%    Number of nodes sampled, 
%    Connectivity Radius of the graph
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph
% Code assumes number of sampled nodes is at least 2 and that total number of nodes is at least 3

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Define colors to draw nodes and edges of the graph
\definecolor{EdgeColor}{rgb}{0.9, 0.9, 0.9}  % Light gray
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, 
                       draw, 
%                       clip = {(\OffsetXLocal,\OffsetYLocal) rectangle (0.2,0.2)},
                       minimum width = \NodeSizeLocal pt,
                       opacity = 0.2,
                       inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraph}[5]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\def\NrNodesLocal           {#1} 
\def\ConnectivityRadiusLocal{#2}
\def\OffsetXLocal           {#3}
\def\OffsetYLocal           {#4}
\def\NodeSizeLocal          {#5}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Draw circle to represent the first graph node. 
% The first node is drawn close to the south east corner 
\pgfmathsetmacro \randX{\Xscale*(1 - 0.1)} % The x-coordinate of node 1
\pgfmathsetmacro \randY{\Yscale*(0 + 0.1)} % The y-coordinate of node 1
\pgfmathsetmacro \posX{\randX + \OffsetXLocal} % Have to move coordinates to offset position of graph
\pgfmathsetmacro \posY{\randY + \OffsetYLocal}
% Draw the node. We use the node layer. This has to be created outside of the macro as it
% needs to be global. NodeLayer must be on top of EdgeLayer.
\begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
   \ChooseNodeColor{\randX}{\randY}   % Choose color for node 
   \node[ GraphNode,                  % Draw the node using GraphNode specifications
          CurrentColor,               % Color for node border
          fill=CurrentColor]          % Color for node interior
          (a1)                        % Node label for future reference
          at (\posX cm, \posY cm) {}; % Node position
\end{pgfonlayer}       

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes that are sampled
% Since node 1 has been drawn, we sweep from 2 to NrNodesSampled nodes.
% We draw random points in the graph box 
%
\foreach \i in {1,...,\NrNodesLocal} 
{
   % Chose node position at random
   \pgfmathsetmacro \randX{\Xscale*rnd} % The x-coordinate of node 1
   \pgfmathsetmacro \randY{\Yscale*rnd} % The y-coordinate of node 1
   \pgfmathsetmacro \posX{\randX + \OffsetXLocal } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \OffsetYLocal }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      \ChooseNodeColor{\randX}{\randY}   % Choose color for node 
      \node[ GraphNode,                  % Draw the node using GraphNode specifications
          CurrentColor,               % Color for node border
          fill=CurrentColor]          % Color for node interior
          (a\i)                        % Node label for future reference
          at (\posX cm, \posY cm) {}; % Node position   
\end{pgfonlayer}       
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin loop for drawing graph edges. 
%% We sweep from 1 to NrNodes drawing random edges
%%
\foreach \i in {2,...,\NrNodesLocal} 
{
   % Draw node connections. We sweep through all past nodes and check if they are close
   % If the nodes are close, we draw an edge.
   \begin{pgfonlayer}{EdgeLayer} % Edges are drawn in the edge layer
      \gettikzxy{(a\i)}{\NodePosX}{\NodePosY}; % Get coordinates of current node (node i)
      \pgfmathsetmacro\PreviousNode{\i -1} % A pgf technicality. Need to store index of previous node (\i-1)
      \foreach \j in {1,...,\PreviousNode} % Start loop sweeping through previous nodes
      {
         \gettikzxy{(a\j)}{\OtherNodePosX}{\OtherNodePosY}; % Coordinates of the other node (node j)
         \CalculateDistance{\NodePosX-\OtherNodePosX}
                           {\NodePosY-\OtherNodePosY}; % Calculate distance between nodes i and j
         \ifdim \Distance cm < \ConnectivityRadiusLocal cm % Check the nodes are close. 
            \draw[EdgeColor] (a\i) -- (a\j); %If they are close, draw and edge
         \fi 
      } % Close inner loop sweeping through previous nodes
   \end{pgfonlayer}      
} % Close main loop sweeping through nodes

} % Close Macro

==> figures/graph_drawing_experiments/old/DrawGraphArray.tex <==
% Command to draw a random graph. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The Edge color is hard coded to light gray
% The size and shape of the node is also hard coded. They are 5pt circles

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The parameters passed to the macro are, in order: 
%    Number of nodes, 
%    Connectivity Radius of the graph
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph
% Code assumes number of sampled nodes is at least 2 and that total number of nodes is at least 3

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Define colors to draw nodes and edges of the graph
\definecolor{EdgeColor}{rgb}{0.9, 0.9, 0.9}  % Light gray
% Define scale of the graph
\def\Xscale{1.5}
\def\Yscale{1}
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, 
                       draw, 
                       minimum width = \NodeSizeLocal pt,
                       opacity = 0.8,
                       inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphArray}[5]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\def\NrNodesLocal           {#1} 
\def\ConnectivityRadiusLocal{#2}
\def\OffsetXLocal           {#3}
\def\OffsetYLocal           {#4}
\def\NodeSizeLocal          {#5}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes that are sampled
% We sweep from 1 to NrNodesSampled nodes.
% We draw random points in the graph box 
%
\foreach \i in {1,...,\NrNodesLocal} 
{
   % Chose node position at random
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \OffsetXLocal } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \OffsetYLocal }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      \ChooseNodeColor{\randX}{\randY}   % Choose color for node 
      \node[ GraphNode,                  % Draw the node using GraphNode specifications
             CurrentColor,               % Color for node border
             fill=CurrentColor]          % Color for node interior
             (a\i)                        % Node label for future reference
             at (\posX cm, \posY cm) {}; % Node position   
\end{pgfonlayer}       
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin loop for drawing graph edges. 
%% We sweep from 1 to NrNodes drawing random edges
%%
\foreach \i in {2,...,\NrNodesLocal} 
{
   % Draw node connections. We sweep through all past nodes and check if they are close
   % If the nodes are close, we draw an edge.
   \begin{pgfonlayer}{EdgeLayer} % Edges are drawn in the edge layer
      \gettikzxy{(a\i)}{\NodePosX}{\NodePosY}; % Get coordinates of current node (node i)
      \pgfmathsetmacro\PreviousNode{\i -1} % A pgf technicality. Need to store index of previous node (\i-1)
      \foreach \j in {1,...,\PreviousNode} % Start loop sweeping through previous nodes
      {
         \gettikzxy{(a\j)}{\OtherNodePosX}{\OtherNodePosY}; % Coordinates of the other node (node j)
         \CalculateDistance{\NodePosX-\OtherNodePosX}
                           {\NodePosY-\OtherNodePosY}; % Calculate distance between nodes i and j
         \ifdim \Distance cm < \ConnectivityRadiusLocal cm % Check the nodes are close. 
            \draw[EdgeColor] (a\i) -- (a\j); %If they are close, draw and edge
         \fi 
      } % Close inner loop sweeping through previous nodes
   \end{pgfonlayer}      
} % Close main loop sweeping through nodes

} % Close Macrozimulitus

==> figures/tikz_styles.tex <==
\tikzstyle{phantom vertex} = [ ellipse, 
                               anchor = center, 
                               minimum height = 0.06*\unit, 
                               minimum width  = 0.06*\unit,
                               inner sep=0pt,
                               anchor=center]
\tikzstyle{red vertex}   = [black, fill = red!20,   phantom vertex, draw]
\tikzstyle{black vertex} = [black, fill = black!20, phantom vertex, draw]
\tikzstyle{blue vertex}  = [black, fill = blue!20,  phantom vertex, draw]
\tikzstyle{green vertex} = [black, fill = green!20,  phantom vertex, draw]
\tikzstyle{vertex}       = [draw, phantom vertex]

\tikzstyle{point} = [ellipse, inner sep=0pt, draw, fill=white, anchor = center,
                     minimum height = 0.05*\unit, minimum width  = 0.05*\unit]

==> figures/toolscnngs/AuxMacrosDrawEdges.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro for computing distance between 2 points

\newcommand{\CalculateDistance}[2]
{
   \pgfmathsetmacro\Distance{ sqrt(     (#1)^2 +    (#2)^2 ) }; % Calculates 2-norm distance
%  \pgfmathsetmacro\Distance{      abs( (#1)   + abs(#2)   ) }; % Calculates 1-norm distance. May be faster
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macro to get coordniates of a node
\makeatletter
\newcommand{\GetTikzXY}[3]{ 
    \tikz@scan@one@point\pgfutil@firstofone#1\relax
    \edef#2{\the\pgf@x}
    \edef#3{\the\pgf@y}
}
\makeatother



==> figures/toolscnngs/ChooseNodeColor.tex <==

% Macro for selecting node's color based on positions. The macro is not used in the final version. 
% Accepts as argument the (x,y) coordinate of the node.
% Returns the custom color currentcolor that can be used in color commands.

\newcommand{\ChooseNodeColor}[2]
{   
    % Store arguments of the function in readable variables
    \def\Xhere{#1}      
    \def\Yhere{#1}
    % Compute a color scale
    \pgfmathsetmacro{\thecurrentcolor}
                    { 0.8*exp( - 0.6*(abs(\Xhere-0.5) + abs(\Yhere-0.5)) }
    % Assign color scale according to colormap (Grayscale in current configuration}
    \definecolor{CurrentColor}{rgb}{\thecurrentcolor,\thecurrentcolor,\thecurrentcolor}
}



%\def\colors{{"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", 
%             "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%             "E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", 
%             "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%             "D5EAE7", "F3ELEB", "F6C4E1", "F79CD4"}} 
%
%\pgfmathsetmacro{\thecurrentcolor}{\colors[random(0,20)]}
%\definecolor{currentcolor}{HTML}{\thecurrentcolor}


==> figures/toolscnngs/DrawFeatures.tex <==

% Macro to draw a stack of features. 
% The first two parameters are the positions of the front feature. 
% The third and fourth two are the x and y offsets of subsequent features. 
% The fifth and sixth are the size of the features 
% The seventh parameter is the number of features
% The eight is the color of the feature plane

\newcommand{\DrawFeatures}[8]
{
   \pgfmathsetmacro\NumberFeatures {#7}    % The numb er of features is in the seventh parameter
   \foreach \i in {\NumberFeatures,...,1}  % Repeat number of features. Sweep backwards
   {
      \pgfmathsetmacro\FeaturePosX {(#3)*(\i-1)} % Offset x
      \pgfmathsetmacro\FeaturePosY {(#4)*(\i-1)} % Offset y  
      \path (#1,           #2)          % Start position
            ++ (\FeaturePosX,\FeaturePosY) % Advance as per offset
       node[draw, 
             rectangle, 
             black!70,
             anchor         = south west,
             fill           = #8, 
             minimum width  = #5,
             minimum height = #6    ]  {} ;
   }
}


==> figures/toolscnngs/DrawGraphEdges.tex <==
% Command to draw edges of a graph. The macro assumes that nodes have been 
% placed and that they have received tikZ labels of the form (a1), (a2), ..., (aN)
% This can be accomplished by loading the file DrawGraphNodes.tex:
%    \input{DrawGraphNodes.tex}
% and calling the macro DrawGraphNodes. The statement below draws nodes of a
% graph with 10 nodes and small circles for nodes:
%    \DrawGraphNodes {1}    % Start node
%                    {10}   % End node 
%                    {5}    % Node size
%                    {1}    % Opacity
%                    {0}    % X offset
%                    {0}    % Y offset

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    NrNodes: Number of nodes the graph has
%    Connectivity radius: How far aways to connect nodes  
%    Edge Color: A valid color to draw edges. E.g., gray!20.
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Load macros to get coordinate points and calculate distances
%
\input{../ToolsCNNGS/AuxMacrosDrawEdges}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphEdges}[7]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNrNodes     {#3}
\pgfmathsetmacro\localRadius      {#4}
\pgfmathsetmacro\localEdgeColor   {#5}
\pgfmathsetmacro\localOffsetX     {#6}
\pgfmathsetmacro\localOffsetY     {#7}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin loop for drawing graph edges. 
%% We sweep from \localStartNode to NrNodes drawing edges
%%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Draw node connections. We sweep through all nodes and check if they are close to \i
   % If the nodes are close, we draw an edge.
   \begin{pgfonlayer}{EdgeLayer} % Edges are drawn in the edge layer
      \GetTikzXY{(a\i)}{\NodePosX}{\NodePosY}; % Get coordinates of current node (node i)
      \pgfmathsetmacro\PreviousNode{\i -1} % A pgf technicality. Need to store index of previous node (\i-1)
      \foreach \j in {1,...,\localNrNodes} % Start loop sweeping through previous nodes
      {
         \GetTikzXY{(a\j)}{\OtherNodePosX}{\OtherNodePosY}; % Coordinates of the other node (node j)
         \CalculateDistance{\NodePosX-\OtherNodePosX}
                           {\NodePosY-\OtherNodePosY}; % Calculate distance between nodes i and j
         \ifdim \Distance cm < \localRadius cm % Check the nodes are close. 
            \draw[\localEdgeColor] (a\i) -- (a\j); %If they are close, draw and edge
         \fi 
      } % Close inner loop sweeping through previous nodes
   \end{pgfonlayer}      
} % Close main loop sweeping through nodes
}
 


==> figures/toolscnngs/DrawGraphNodes.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodes}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired
      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position 
     \clip  (-0.1,-0.1) rectangle (\Xscale + 0.1, \Yscale + 0.1);
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity]    % Node opacity
             (\posX cm, \posY cm)            % Node position
             circle (\localNodeSize pt);     % Node size

\end{pgfonlayer}       
}
}


==> figures/toolscnngs/DrawGraphNodesR.tex <==
% Command to draw the nodes of a graph with coordinates pre-specified in 
% coordinate arrays \posXarray and \posYarray. 
% The dimensions of the graph are hard coded to 1.5 by 1. 
% The shape of the node is also hard coded. They are 5pt circles.

% The macro requires prior definition of coordinate arrays \posXarray and \posYarray
% I have 200 stored coordinates in the file:
%    \input{NodePositions.tex}

% The macro assumes that the dimensions of the graph have been specified.
% This requires that we define variables \Xscale and \Yscale
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The macro assumes existence of a function \ChooseNodeColor{X}{Y} that will
% define the custom color CurrentColor which is used to choose the color of
% a node at coordinates (X,Y). This can be accomplished by loading:
%    \input{ChooseNodeColor.tex}
% Alternatively, colors cab be preloaded on an array. This array is called 
% \NodeColors and it is currently stored in NodePositions.tex. Current compilation
% uses color array. This can be changed by uncommenting a line below.

% The macro requires prior definition of at least two pgflayers for nodes and edges.
% The Node Layer must be on top of the Edge Layer so that nodes override edges.
% This is accomplished by adding the commands:
%    \pgfdeclarelayer{NodeLayer}
%    \pgfdeclarelayer{EdgeLayer}
%    \pgfsetlayers   {EdgeLayer,NodeLayer}
% This is not done here in case there is a need to add more layers

% The macro also requires outside definition of the graph scale. This can be 
% done by adding the commands
%    \def\Xscale{1.5}
%    \def\Yscale{1}

% The parameters passed to the macro are, in order: 
%    Start Node: First node to draw (between 1 and 199)
%    End Node: Last node to draw (between (2 and 200, strictly larger than Start Node)
%    Node Size: How large the nodes are
%    Node Opacity: Reduce number towards 0 to dim the brightness of the node
%    x-Offset to move the graph around. This is the south coordinate for location of the graph
%    y-Offset to move the graph around. This is the west coordinate for location of the graph

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hard coded specifications
%
% Specifications of for the shape and size of a node
\tikzstyle{GraphNode}=[circle, inner sep = 0]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Macro
%
\newcommand{\DrawGraphNodesR}[6]{

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convert parameters to readable variables
%
\pgfmathsetmacro\localStartNode   {#1} 
\pgfmathsetmacro\localEndNode     {#2}
\pgfmathsetmacro\localNodeSize    {#3}
\pgfmathsetmacro\localNodeOpacity {#4}
\pgfmathsetmacro\localOffsetX     {#5}
\pgfmathsetmacro\localOffsetY     {#6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin loop for drawing the graph nodes 
% We sweep from Start Node to End Node
% We read coordinates from \posXarray and \posYarray
%
\foreach \i in {\localStartNode,...,\localEndNode} 
{
   % Chose node position from \posXarray and \posYarray
   \pgfmathsetmacro \randX{\Xscale*\posXarray[\i-1]}   
   \pgfmathsetmacro \randY{\Yscale*\posYarray[\i-1]}
   \pgfmathsetmacro \posX{\randX + \localOffsetX } % Have to move coordinates to offset position of graph
   \pgfmathsetmacro \posY{\randY + \localOffsetY }
   % Draw circle to represent graph node. We used the node layer. This has to be created outside 
   % of the macro as it needs to be global. NodeLayer must be on top of EdgeLayer.
   \begin{pgfonlayer}{NodeLayer} % Edges are drawn in the node layer
      %\ChooseNodeColor{\randX}{\randY}       % Choose color for node using macro. Uncomment if desired
      \pgfmathsetmacro{\thecurrentcolor} {\NodeColors[\i-1]} % Choose color from color array. Comment if desired
      \definecolor{CurrentColor}{HTML}{\thecurrentcolor}     % Define color. Comment if desired
      \node  [ GraphNode ]                   % Draw the node using GraphNode specifications
             (a\i)                           % Node label for future reference
             at (\posX cm, \posY cm) {};     % Node position 
     \clip  (-0.1,-0.1) rectangle (1.6, 1.1);
      \path[ CurrentColor,                   % Color for node border
             %inner color=CurrentColor,      % Uncomment for radial color gradient
             %outer color=FeaturePlaneColor, % Uncomment for radial color gradient
             fill = CurrentColor,            % Color for node interior
             opacity = \localNodeOpacity,    % Node opacity
             rounded corners]
             (\posX cm - \localNodeSize pt, \posY cm - \localNodeSize pt)            % Node position
             rectangle (\posX cm + \localNodeSize pt, \posY cm + \localNodeSize pt);     % Node size

\end{pgfonlayer}       
}
}


==> figures/toolscnngs/palettes/alejandro.tex <==
\def \NodeColors{{
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
%"023FA5", "7D87B9", "BEC1D4", "D6BCC0", "BB7784", "8E063B", "4A6FE3", "8595E1", "B5BBE3", "E6AFB9",
%"E07B91", "D33F6A", "11C638", "8DD593", "C6DEC7", "EAD3C6", "F0B98D", "EF9708", "0FCFC0", "9CDED6",
}} 


==> figures/toolscnngs/palettes/w3schools.tex <==
\def \NodeColors{{
"A9A904", "2EA904", "A90404", "A92E04", "A95704", "A98004", "80A904", "57A904",  "04A904", "04A92E",
"04A957", "04A980", "04A9A9", "0480A9", "045EA7", "0457A9", "042EA9", "0404A9", "2E04A9", "5704A9",
"8004A9", "A904A9", "A90480", "A90457", "A9042E", 
"A90404", "A92E04", "A95704", "A98004", "A9A904", "80A904", "57A904", "2EA904", "04A904", "04A92E",
"04A957", "04A980", "04A9A9", "0480A9", "045EA7", "0457A9", "042EA9", "0404A9", "2E04A9", "5704A9",
"8004A9", "A904A9", "A90480", "A90457", "A9042E",
"A90404", "A92E04", "A95704", "A98004", "A9A904", "80A904", "57A904", "2EA904", "04A904", "04A92E",
"04A957", "04A980", "04A9A9", "0480A9", "045EA7", "0457A9", "042EA9", "0404A9", "2E04A9", "5704A9",
"8004A9", "A904A9", "A90480", "A90457", "A9042E",
"A90404", "A92E04", "A95704", "A98004", "A9A904", "80A904", "57A904", "2EA904", "04A904", "04A92E",
"04A957", "04A980", "04A9A9", "0480A9", "045EA7", "0457A9", "042EA9", "0404A9", "2E04A9", "5704A9",
"8004A9", "A904A9", "A90480", "A90457", "A9042E",
}} 


==> gated_proof.tex <==
\subsection{Stability} \label{subsec:gatingStability}

\blue{Since the parameters of the gate operators $\hcalQ$ and $\kcalQ$ are themselves the outputs of GRNNs, it is natural to ask whether the stability result from Theorem \ref{thm:stability} carries over to the gated GRNN in \eqref{eqn:gatingGeneric}. In order to analyze its stability without focusing on a specific type of gating, we will describe the
parameters of $\hcalQ$ and $\kcalQ$ as $\hat{\bbtheta}$ and $\check{\bbtheta}$, and the architectures used to predict these parameters from the state variables $\hbz_t$ \eqref{eqn:inputgatestate} and $\cbz_t$ \eqref{eqn:forgetgatestate} as generic models $\hat{\bbPhi}_{\bbS}$ and $\check{\bbPhi}_\bbS$ (the subscript $\bbS$ indicates that the graph is a hyperparameter). Strictly speaking, the parameters of the input and forget gates are obtained as $\hat{\bbtheta} = \hat{\bbPhi}_\bbS(\hbz_t)$ and $\check{\bbtheta} = \check{\bbPhi}_\bbS(\cbz_t)$, and we can write $\hcalQ = \hcalQ_{\hat{\bbtheta}}$ and $\kcalQ = \kcalQ_{\check{\bbtheta}}$. Note that the generic architectures $\hat{\bbPhi}_\bbS$ and $\check{\bbPhi}_\bbS$ can always be particularized to different gating mechanisms. In the case of time gating, $\hat{\bbPhi}_\bbS$ and $\check{\bbPhi}_\bbS$ are fully connected layers and $\hat{\bbtheta}$, $\check{\bbtheta}$ are scalars [cf. \eqref{eqn:tgates_comp}]; in node gating, $\hat{\bbPhi}_\bbS$ and $\check{\bbPhi}_\bbS$ are GNNs and $\hat{\bbtheta}$, $\check{\bbtheta}$ are vectors [cf. \eqref{eqn:ngates_comp}]; and, in edge gating, $\hat{\bbPhi}_\bbS$ and $\check{\bbPhi}_\bbS$ are the attention mechanism of a GAN and $\hat{\bbtheta}$, $\check{\bbtheta}$ are matrices [cf. \eqref{eqn:edgeGateComps}]. 
%The benefit of this generic representation is that, regardless of the type of gating, we can write the operator norms of the input and forget gates as
%\begin{align}
%\begin{split}
%\|\hcalQ\| &= \|\hat{\bbPhi}(\hbZ_t)\| \\
%\|\kcalQ\| &= \|\check{\bbPhi}(\cbZ_t)\|.
%\end{split}
%\end{align}

To prove stability of gated GRNNs, we also need the following assumptions on the gate operators $\hcalQ$, $\kcalQ$ and on the parameter learning models ${\hat{\bbPhi}_\bbS}$, $\check{\bbPhi}_\bbS$.

\begin{assumption} \label{as5}
In the induced operator norm, the operators $\hcalQ=\hcalQ_{\hat{\bbtheta}}$ and $\kcalQ=\kcalQ_{\check{\bbtheta}}$ are $Q$-Lipschitz with respect to $\hat{\bbtheta}$ and $\check{\bbtheta}$, i.e. $\|\hcalQ_{\hat{\bbtheta}^{(1)}}-\hcalQ_{\hat{\bbtheta}^{(2)}}\| \leq Q\|\hat{\bbtheta}^{(1)}-\hat{\bbtheta}^{(2)}\|$.
\end{assumption}
 
\begin{assumption} \label{as6}
The models ${\hat{\bbPhi}_\bbS}$ and $\check{\bbPhi}_\bbS$ are $\phi_1$-Lipschitz with respect to $\hbZ_t$ and $\cbZ_t$, i.e. $\|{\hat{\bbPhi}}_\bbS(\hbz^{(1)}_t) - {\hat{\bbPhi}}_\bbS(\hbz^{(2)}_t)\| \leq \phi_1 \|\hbz^{(1)}_t-\hbz^{(2)}_t\|$.
\end{assumption}

\begin{assumption} \label{as7}
In the induced operator norm, the models ${\hat{\bbPhi}_\bbS}$ and $\check{\bbPhi}_\bbS$ are $\phi_2$-Lipschitz with respect to the graph, i.e. $\|{\hat{\bbPhi}}_{\bbS^{(1)}} - {\hat{\bbPhi}}_{\bbS^{(2)}}\| \leq \phi_2 \|\bbS^{(1)}-\bbS^{(2)}\|$.
\end{assumption}

Assumption \ref{as5} is important because it allows expressing the norm of the difference operator in terms of the norm difference of the operators' parameters. It is also worth noting that Assumptions \ref{as6} and \ref{as7} are not too restrictive, as we discuss in more detail in Remark \ref{rmk:restrictive}.  

\begin{theorem} \label{thm:GGRNNstability}
\end{theorem}

We observe that...

\begin{remark} \label {rmk:restrictive}
Fully connected and convolutional layers with most conventional activation functions are Lipschitz stable to input perturbations \cite{X}, so Assumption \ref{as6} is generally satisfied for all types of gating (in edge gating, the most common attention mechanism is a multi-layer perceptron \cite{Velickovic18-GraphAttentionNetworks}). In the case of time gating, the fully connected layers that make up $\hat{\bbPhi}$ and $\check{\bbPhi}$ do not depend on $\bbS$, so Assumption \ref{as7} is also satisfied automatically. Since in node gating $\hat{\bbPhi}$ and $\check{\bbPhi}$ are GNNs, Assumption \ref{as7} is guaranteed by \cite[Theorem X]{Gama19-Stability} as long as the graph convolutions are integral Lipschitz [cf. Definition \ref{def:integralLipschitz}] and the activation functions are normalized Lipschitz [cf. Assumption \ref{as2}]. 
Finally, we can expect Assumption \ref{as7} to hold for edge gating at least in cases where the edges of the graph are preserved, since the attention coefficients only depend on there being an edge between two nodes, but not on the edge weight. Note that edge preservation is generally enforced by the definition of the minimum relative perturbation matrix, which measures how close two graphs are from being permutations of one another  [cf. \eqref{eqn:graphDistance}].
\end{remark}

}

\section{Proof of Theorem 2} \label{sec:appendixC}
\blue{
\begin{proof}[Proof of Theorem \ref{thm:GGRNNstability}]
To simplify notation, we will write the input and forget gate operators whose parameters $\hat{\bbtheta}$ and $\check{\bbtheta}$ have been perturbed as
\begin{align}
\begin{split}
\hcalQ_{\tilde{\hat{\bbtheta}}} &= \tilde{\hcalQ}\\
\kcalQ_{\tilde{\check{\bbtheta}}} &= \tilde{\kcalQ}.
\end{split}
\end{align}

By the same reasoning used in equations \eqref{eqn:output_diff1} and \eqref{eqn:output_diff1.1} of the proof of Theorem \ref{thm:stability}, we start by bounding $\|\bby_t-\tby_t\|$ as
\begin{align} \label{eqn:thm2_output_diff1.1}
\|\bby_t - \tilde{\bby}_t\| \leq \|\bbC\|\|\bbz_t-\tbz_t\| + \|\bbC-\tbC\|\|\tbz_t\|\text{.}
\end{align}
%The norm of $\bbC$ is assumed bounded, and Lemma \ref{lemmaStab} gives a bound to $\|\bbC-\tbC\|$.
Using \eqref{eqn:gatingGeneric} and the fact that $\sigma$ is normalized Lipschitz, we can write
\begin{align} \label{eqn:thm2_state_diff1}
\begin{split}
\|\bbz_t-\tbz_t\| =&\ \|\sigma(\hcalQ(\bbA\bbx_t)+\kcalQ(\bbB\bbz_{t-1}))\\
&-\sigma(\tilde{\hcalQ}(\tbA\bbx_t)+\tilde{\kcalQ}(\tbB\tbz_{t-1}))\| \\
&\leq \|\hcalQ(\bbA\bbx_t)-\tilde{\hcalQ}(\tbA\bbx_t)\| \\
&+\|\kcalQ(\bbB\bbz_{t-1})-\tilde{\kcalQ}(\tbB\tbz_{t-1})\| 
\end{split}
\end{align} 
where the bound follows from the triangle inequality.
Focusing on the first term on the right-hand side of \eqref{eqn:thm2_state_diff1}, we apply the triangle once again to get
\begin{align} \label{eqn:thm2_state_diff1.1}
\begin{split}
\|\hcalQ&(\bbA\bbx_t)-\tilde{\hcalQ}(\tbA\bbx_t)\| =\\
&= \|\hcalQ(\bbA\bbx_t)+\tilde{\hcalQ}(\bbA\bbx_t)-\tilde{\hcalQ}(\bbA\bbx_t)-\tilde{\hcalQ}(\tbA\bbx_t)\| \\
&\leq \|\hcalQ(\bbA\bbx_t)-\tilde{\hcalQ}(\bbA\bbx_t)\| +\|\tilde{\hcalQ}(\bbA\bbx_t)-\tilde{\hcalQ}(\tbA\bbx_t)\|.
\end{split}
\end{align}
Using the Cauchy-Schwarz inequality and Assumption \ref{as5} lets us write
\begin{align} \label{eqn:1.1}
\begin{split}
\|\hcalQ(\bbA\bbx_t)-\tilde{\hcalQ}(\bbA\bbx_t)\| \leq \|\hcalQ-\tilde{\hcalQ}\|\|\bbA\|\|\bbx_t\| \\
\leq Q\|\hat{\bbPhi}_\bbS(\hbz_t)-\hat{\bbPhi}_\tbS(\tilde{\hbz}_t)\|\|\bbA\|\|\bbx_t\|
\end{split}
\end{align}
and, adding and subtracting $\hat{\bbPhi}_\tbS(\hbz_t)$ to $\|\hat{\bbPhi}_\bbS(\hbz_t)-\hat{\bbPhi}_\tbS(\tilde{\hbz}_t)\|$ and applying the triangle inequality,
\begin{align} \label{eqn:1.1.1}
\begin{split}
\|\hat{\bbPhi}_\bbS&(\hbz_t)-\hat{\bbPhi}_\tbS(\tilde{\hbz}_t)\| \\
&\leq \|\hat{\bbPhi}_\bbS(\hbz_t)-\hat{\bbPhi}_\tbS(\hbz_t)\| + \|\hat{\bbPhi}_\tbS(\hbz_t)-\hat{\bbPhi}_\tbS(\tilde{\hbz}_t)\| \\
&\leq \phi_2 \varepsilon \|\hbz_t\| + \phi_1 \|\hbz_t -\tilde{\hbz}_t\|
\end{split}
\end{align}
where the second inequality follows from Assumptions \ref{as6} and \ref{as7}.

To bound the second term on the right-hand side of \eqref{eqn:thm2_state_diff1.1}, we use the fact that the gate operator is additive. Explicitly,
\begin{align} \label{eqn:1.2}
\begin{split}
\|\tilde{\hcalQ}(\bbA\bbx_t)-\tilde{\hcalQ}(\tbA\bbx_t)\| &= \|\tilde{\hcalQ}(\bbA\bbx_t-\tbA\bbx_t)\| \\
&\leq \|\bbA-\tbA\|\|\bbx_t\|
\end{split}
\end{align}
where we have used the Cauchy-Schwarz inequality and the fact that $\|\tilde{\hcalQ}\|\leq 1$. Putting equations \eqref{eqn:1.1}, \eqref{eqn:1.1.1} and \eqref{eqn:1.2}, we arrive at a bound for $\|\hcalQ(\bbA\bbx_t)-\tilde{\hcalQ}(\tbA\bbx_t)\|$,
\begin{align} \label{eqn:1}
\begin{split}
\|\hcalQ(\bbA\bbx_t)&-\tilde{\hcalQ}(\tbA\bbx_t)\|
\leq Q\phi_2\varepsilon\|\hbz_t\|\\
&+ Q\phi_1\|\hbz_t-\tilde{\hbz}_t\| + \|\bbA-\tbA\|
\end{split}
\end{align}
where we have additionally used Assumptions \ref{as1} and \ref{as4} to bound $\|\bbA\|$ and $\|\bbx_t\|$. 

Moving onto the second term on the right-hand side of \eqref{eqn:thm2_state_diff1}, we add and subtract $\tilde{\kcalQ}(\bbB\bbz_{t-1})$ and use the triangle inequality to get 
\begin{align} 
\begin{split}
\|\kcalQ(\bbB\bbz_{t-1})-&\tilde{\kcalQ}(\tbB\tbz_{t-1})\| \leq \\
&\leq \|\kcalQ(\bbB\bbz_{t-1})-\tilde{\kcalQ}(\bbB\bbz_{t-1})\| \\
&+ \|\tilde{\kcalQ}(\bbB\bbz_{t-1})-\tilde{\kcalQ}(\tbB\tbz_{t-1})\|.
\end{split}
\end{align}
Using the Cauchy-Schwarz inequality and Assumption \ref{as5},
\begin{align} \label{eqn:2.1}
\begin{split}
\|\kcalQ(\bbB\bbz_{t-1})-&\tilde{\kcalQ}(\bbB\bbz_{t-1})\| \leq \\
&\leq \|\kcalQ-\tilde{\kcalQ}\|\|\bbB\|\|\bbz_{t-1}\| \\
&\leq Q\|\check{\bbPhi}_\bbS(\cbz_{t})-\check{\bbPhi}_\tbS(\tilde{\cbz}_{t})\|\|\bbB\|\|\bbz_{t-1}\|
\end{split}
\end{align}
and adding and subtracting $\check{\bbPhi}_\tbS(\cbz_t)$ to $\|\check{\bbPhi}_\bbS(\cbz_{t})-\check{\bbPhi}_\tbS(\tilde{\cbz}_{t})\|$ like in \eqref{eqn:1.1.1},
\begin{align} \label{eqn:2.1.1}
\|\check{\bbPhi}_\bbS(\cbz_{t})-\check{\bbPhi}_\tbS(\tilde{\cbz}_{t})\| \leq \phi_2 \varepsilon \|\cbz_t\| + \phi_1 \|\cbz_t -\tilde{\cbz}_t\|.
\end{align}

To bound $\|\tilde{\kcalQ}(\bbB\bbz_{t-1})-\tilde{\kcalQ}(\tbB\tbz_{t-1})\|$, we use the fact that the gating operator is additive and bounded by $1$ to write
\begin{align} \label{eqn:2.2}
\begin{split}
\|\tilde{\kcalQ}(\bbB\bbz_{t-1})-\tilde{\kcalQ}(\tbB\tbz_{t-1})\| &= \|\tilde{\kcalQ}(\bbB\bbz_{t-1}-\tbB\tbz_{t-1})\| \\
&\leq \|\tilde{\kcalQ}\|\|\bbB\bbz_{t-1}-\tbB\tbz_{t-1}\| \\
&\leq \|\bbB\bbz_{t-1}-\tbB\tbz_{t-1}\|
\end{split}
\end{align}
where the first inequality follows from Cauchy-Schwarz. Finally, adding and subtracting $\tbB\bbz_{t-1}$ to $\|\bbB\bbz_{t-1}-\tbB\tbz_{t-1}\|$ and applying the triangle and Cauchy-Schwarz inequalities, we get
\begin{align} \label{eqn:2.2.1}
\|\bbB\bbz_{t-1}-\tbB\tbz_{t-1}\| \leq \|\bbB-\tbB\|\|\bbz_{t-1}\|+\|\tbB\|\|\bbz_{t-1}-\tbz_{t-1}\| 
\end{align}
and putting together equations \eqref{eqn:2.1} through \eqref{eqn:2.2.1}, we arrive at a bound for $\|\kcalQ(\bbB\bbz_{t-1})-\tilde{\kcalQ}(\tbB\tbz_{t-1})\|$ given by
\begin{align} \label{eqn:2}
\begin{split}
\|\kcalQ(&\bbB\bbz_{t-1})-\tilde{\kcalQ}(\tbB\tbz_{t-1})\| \leq Q\phi_2\varepsilon \|\cbz_t\|\|\bbz_{t-1}\|\\
&+Q\phi_1\|\cbz_t-\tilde{\cbz}_t\|\|\bbz_{t-1}\|+\|\bbB-\tbB\|\|\bbz_{t-1}\|\\
&+\|\bbz_{t-1}-\tbz_{t-1}\|.
\end{split}
\end{align}

Plugging \eqref{eqn:1} and \eqref{eqn:2} back in \eqref{eqn:thm2_state_diff1}, we arrive at a recurrence relationship for $\|\bbz_t-\tbz_t\|$. Explicitly,
\begin{align} \label{eqn:thm2_recurrence}
\begin{split}
\|\bbz_t-\tbz_t\| &\leq \|\bbz_{t-1}-\tbz_{t-1}\| + Q\phi_2\varepsilon\|\hbz_t\| \\
&+ Q\phi_1\|\hbz_t-\tilde{\hbz}_t\|
+ \|\bbA-\tbA\| \\
&+  \|\bbz_{t-1}\|Q(\phi_2\varepsilon \|\cbz_t\|
+\phi_1\|\cbz_t-\tilde{\cbz}_t\|) \\
&+ \|\bbz_{t-1}\|\|\bbB-\tbB\|.
\end{split}
\end{align}
Note that, because the GRNN used to compute the input gate state $\hbz_t$ is not gated, we can use equations \eqref{eqn:bound_nongated_state} and \eqref{eqn:state_diff3} to solve this recursion for the second and third terms on the right-hand side, which only depend on $\|\hbz_t\|$ and $\|\hbz_t-\tilde{\hbz}_t\|$. We also know bounds for $\|\cbz_t\|$ and $\|\cbz_t-\tilde{\cbz}_t\|$, but the last two terms of \eqref{eqn:thm2_recurrence} also depend on $\|\bbz_{t-1}\|$. To bound it, we use \eqref{eqn:gatingGeneric} and write
\begin{align}
\|\bbz_i\| &= \|\sigma(\hcalQ(\bbA\bbx_i)+\kcalQ(\bbB\bbz_{i-1}))\| \\
&\leq \|\hcalQ(\bbA\bbx_i)+\kcalQ(\bbB\bbz_{i-1})\| \\
&\leq \|A\|\|\bbx_i\|+\|\bbB\|\|\bbz_{i-1}\|
\end{align}
where the first inequality follows from Assumption \ref{as2} and the second from the Cauchy-Schwarz inequality and the fact that the gate operator norms are bounded by $1$. The hidden state norm $\|\bbz_i\|$ is thus bounded like in \eqref{eqn:bound_nongated_state}.





\end{proof}
}

==> vanishing_gradients.tex <==
When the data sequences that we consider contain long term dependencies, the problem of \textit{vanishing/exploding gradients} may arise \cite{pascanu2013difficulty, bengio1994learning}. For ease of exposition, let $F=H=1$ (equation \eqref{eqn:GRNNhidden}), and let $\bbz_t$ be written as $\bbz_t = \sigma (\bbc_t)$ where $\bbc_t = \bbA(\bbS)\bbx_t + \bbB(\bbS)\bbz_{t-1}$. Denote the loss function by $\ccalL$; if we group all the parameters of $\bbB(\bbS)$ (the state-to-state map) in the parameter tensor $\Theta_\bbB$, the gradient of $\ccalL$ with respect to $\Theta_\bbB$ is given by
\begin{align}
\dfrac{\partial \ccalL}{\partial \Theta_\bbB} &= \sum_{t=1}^T \dfrac{\partial \ccalL_t}{\partial \Theta_\bbB} \\
\dfrac{\partial \ccalL_t}{\partial \Theta_\bbB} &= \sum_{k=1}^t \dfrac{\partial \ccalL_t}{\partial \bbz_t} \dfrac{\partial \bbz_t}{\partial \bbz_k} \dfrac{\partial^+ \bbz_k}{\partial \Theta_\bbB}
\end{align}
where ${\partial^+ \bbz_k}/{\partial \Theta_\bbB}$ denotes the derivative of the evaluation of the state $\bbz_k$ at the $k$th forward propagation step, that is, for a fixed value of the parameters $\Theta_\bbB$ obtained in the preceding backpropagation step.
The partial derivatives $\partial \ccalL_t / \partial \bbz_t$ and ${\partial^+ \bbz_k}/{\partial \Theta_\bbB}$ are easy to compute, so we focus on $\partial \bbz_t / \partial \bbz_k$ for $1 \leq k \leq t$. If we decompose this term by taking partial derivatives with respect to $\bbc_k$, we get
\begin{align} \label{eqn:van_gradients}
\dfrac{\partial \bbz_t}{\partial \bbz_k}  = \dfrac{\partial \bbz_t}{\partial \bbc_t} \dfrac{\partial \bbc_t}{\partial \bbz_{t-1}} \dfrac{\partial \bbz_{t-1}}{\partial \bbc_{t-1}} \dfrac{\partial \bbc_{t-1}}{\partial \bbz_{t-2}} \ldots \\ \dfrac{\partial \bbz_{k+1}}{\partial \bbc_{k+1}} \dfrac{\partial \bbc_{k+1}}{\partial \bbz_{k}} = \prod_{i=k}^t \left( \dfrac{\partial \bbz_i}{\partial \bbc_i} \bbB(\bbS) \right)
\end{align}
where ${\partial \bbz_i}/{\partial \bbc_i}$ is a diagonal matrix whose $j$th diagonal element is given by $d \sigma(c)/ d c |_{c = [\bbc_i]_j}$. We can then see that, for large $t$, the gradient $\partial \ccalL_t / \partial \Theta_\bbB$ depends on successive multiplications by $\bbB(\bbS)$, which is problematic if the eigenvalues of $\bbB(\bbS)$ are too small or too large. If a given eigenvalue of $\bbB(\bbS)$ is much smaller than $1$, the dependencies between $\bbz_t$ and and $\bbz_{t-k}$ along the direction spanned by the corresponding eigenvector will tend to vanish with $t-k$, making it hard to determine the direction where the parameters should move to optimize the loss. Conversely, if this eigenvalue is too large, the gradients in this direction risk exploding and making learning unstable. We refer to this problem as \textit{vanishing/exploding gradients in time}. 

Even if the eigenvalues are not too small or too large, another potential hurdle is the case where some nodes or paths get assigned more importance than others in long range exchanges, leading to a ``spatial imbalance'' and thus making it harder to encode certain graph dependencies. This is because, in fact, the matrix multiplications by $\bbB(\bbS)$ in \eqref{eqn:van_gradients} are actually multiplications by powers of $\bbS^{t-k}$. If the graph has some components that are highly connected, for instance, parts of $\bbS^{t-k}$ might get densely populated for large $t$, overshadowing the local, sparser structures of these connected components and making it harder to encode long term processes that are local on the graph. We call this the problem of \textit{vanishing/exploding gradients in space}.
